Rational curves on fibered varieties

Let $X$ be a projective variety with log terminal singularities and vanishing augmented irregularity. In this paper we prove that if $X$ admits a relatively minimal genus one fibration then it does contain a subvariety of codimension one covered by rational curves contracted by the fibration. We then focus on the case of varieties with numerically trivial canonical bundle and we discuss several consequences of this result.

==> inizioprimocapitolo.tex <==
Even if one is mainly interested in smooth varieties, the natural setting is to allow at least canonical singularities. 

\begin{definition}
	A Calabi-Yau variety is a 
\end{definition}

==> rdivisorinefbig.tex <==

To prove Theorem \ref{newovercurves} we need some basic results.
The well-known statement for $\mathbb{Q}$-divisors that a nef divisor is big if and only if it has positive top self-intersection \cite[Theorem 2.2.13]{lazarsfeld2017positivity1} holds also for $\R$-divisors. This fact is well-known to the experts but we haven't found any references in the literature.



==> teoremasucurve.tex <==

%\begin{remark}
%	By \cite[Theorem 1.17]{greb2016etale}, the intersection of the second Chern class with any $n-2$ ample line bundles is positive.
%\end{remark}

\begin{remark}
	Theorem \ref{sucurve} is a generalization of \cite[Theorem 1.6]{diverio2016rational} also for smooth varieties. Indeed for smooth varieties with trivial canonical bundle with a fibration onto a curve with general fiber an abelian variety $F$, the class of $F$ in $N^1(X)$ has numerical dimension one and intersect in zero the second Chern class of $X$, \textsl{i.e.} $F\cdot c_2(X)=0$ \cite[Section 3]{diverio2016rational}. Moreover a divisor with numerical dimension one wich intersect in zero the second Chern class of $X$ is just conjecturally semiample.
\end{remark}
The geometric meaning of \ref{sucurve} is clear if the divisor is also semiample. In this case the Itaka fibration associated to $D$ is a fibration onto a curve. A general fiber $F$ of such morphism does not intersect $c_2(X)$, \emph{i.e.} $c_2(F)=F\cdot c_2(X)=0$. If $F$ is contained in the regular part of $X$, then by adjunction formula $F$ has automatically trivial canonical bundle. This in particular implies that there is an abelian variety with a finite quasi-\'etale cover to $F$.
%To prove theorem \ref{sucurve} we need some basic results.
